Towards a Unified Understanding of Robot Manipulation: A Comprehensive Survey

Embodied intelligence has witnessed remarkable progress in recent years, driven by advances in computer vision, natural language processing, and the rise of large-scale multimodal models. Among its core challenges, robot manipulation stands out as a fundamental yet intricate problem, requiring the seamless integration of perception, planning, and control to enable interaction within diverse and unstructured environments. This survey presents a comprehensive overview of robotic manipulation, encompassing foundational background, task-organized benchmarks and datasets, and a unified taxonomy of existing methods. We extend the classical division between high-level planning and low-level control by broadening high-level planning to include language, code, motion, affordance, and 3D representations, while introducing a new taxonomy of low-level learning-based control grounded in training paradigms such as input modeling, latent learning, and policy learning. Furthermore, we provide the first dedicated taxonomy of key bottlenecks, focusing on data collection, utilization, and generalization, and conclude with an extensive review of real-world applications. Compared with prior surveys, our work offers both a broader scope and deeper insight, serving as an accessible roadmap for newcomers and a structured reference for experienced researchers. All related resources, including research papers, open-source datasets, and projects, are curated for the community at https://github.com/BaiShuanghao/Awesome-Robotics-Manipulation.

==> sections/5_high-level_planner/affordance_learning.tex <==
% Affordance
% \section{Affordance Learning}
% \label{subsec: affordance_learning}

% A unified understanding of robot manipulation requires moving beyond asking what things are to discerning what can be done with them. The concept of affordance, originating from psychologist J.J. Gibson, provides a powerful framework for this shift~\cite{gibson2014theory}. In robotics, an affordance represents the potential for interaction an object or environment offers relative to a robot's capabilities—a door affords opening, a surface affords placing. By intrinsically linking perception to action, affordances serve as a foundational bridge for building more general and intelligent manipulation systems.

% The study of affordances has evolved from early model-based geometric reasoning to modern data-driven paradigms. The rise of deep learning, in particular, now enables robots to learn functional properties directly from raw sensory data, often through self-supervised interaction. This chapter explores the central role of affordance in this modern context, dissecting the concept from four critical perspectives.

% \subsection{Articulated Object Affordance}
% A significant frontier in robot manipulation is the interaction with articulated objects. Unlike their rigid counterparts, the affordances of objects like cabinets, laptops, and drawers are not merely defined by their static surface properties but are governed by their underlying, often unobservable, kinematic structures. This introduces the challenge of perceiving kinematic affordance: the potential for motion dictated by joints, axes, and constraints. A unified understanding of manipulation must therefore encompass the ability to infer these latent physical properties and translate them into effective interaction strategies.

% A foundational approach to uncovering these hidden kinematics is through physical interaction. By observing an object's state change before and after a manipulation attempt, a robot can infer its articulation model. Ditto~\cite{jiang2022ditto} exemplifies this principle by employing interactive perception to build interactive `digital twins' of real-world objects. From a pair of point cloud observations, Ditto jointly reconstructs part-level geometry and estimates the articulation model (e.g., revolute or prismatic joints), creating a fully-fledged virtual representation that can be instantiated in a physics simulator. This line of work establishes that interaction is a key modality for grounding a robot's understanding of an object's physical possibilities.

% The advent of Large Language and Vision-Language Models (LLMs and VLMs) has catalyzed a paradigm shift, moving from purely geometric reasoning to a synthesis of semantics, physics, and language. These models offer the potential to reason about manipulation in a more human-like, conceptual manner. A key insight is the need to bridge human-defined semantic parts with their physical functionalities. SAGE~\cite{geng2024sage} explicitly addresses this by distinguishing between an object's semantic parts (e.g., a `container') and its actionable parts (e.g., a `pressable button'), fusing the general knowledge of a VLM with the predictions of a domain-specific model to ground instructions. Building on this, other works explore how to effectively communicate kinematic knowledge to LLMs. The framework of Kinematic-aware Prompting~\cite{xia2024kinematic} proposes a unified parser that translates an object's kinematic structure into a structured textual description. This description is then used to prompt an LLM, guiding it to generate a sequence of low-level 3D waypoints for the robot, effectively converting abstract physical knowledge into concrete actions.

% This integration of language and reasoning has paved the way for learning robot-agnostic, object-centric representations that encapsulate affordances more directly. Instead of learning robot-specific actions, these methods aim to predict an intrinsic, actionable model of the object itself. A3VLM~\cite{huang2025a3vlm} pioneers this by training a VLM to predict a compact triad—(Bounding Box, Axis, Semantic Label)—from a single RGB image. This object-centric representation contains all the necessary information for a robot to derive a manipulation policy using simple action primitives. Pushing this concept towards greater generality, UniAff~\cite{yu2025uniaffunifiedrepresentationaffordances} introduces a unified affordance representation for both articulated objects and tools, demonstrating that a single VLM can learn a common functional vocabulary that spans diverse object categories and manipulation tasks.

% Finally, for any manipulation framework to be truly robust in the real world, it must be able to learn from and recover from failure. Recent work has focused on closing the loop through interactive correction. AIC MLLM~\cite{xiong2025autonomous} introduces a system that leverages failed interactions to improve subsequent attempts. When an action fails to produce the desired motion, a feedback module extracts information about the failure—for instance, by generating a visual mask over an unmovable part. This feedback is then used to prompt the MLLM to correct its next SE(3) pose prediction. By incorporating mechanisms for self-reflection and correction, such as Test-Time Adaptation (TTA), the system becomes more resilient and adaptive. This ability to reason about and learn from failure is a crucial component of a unified understanding of manipulation, enabling robots to operate more robustly in complex and unstructured environments.

% \subsection{Part-based Object Affordance}

% A central tenet for achieving a unified understanding of manipulation is the principle of compositionality. Humans effortlessly generalize manipulation skills to novel objects not by memorizing every object's function, but by understanding that objects are assemblies of functional parts. A handle affords grasping, a lid affords opening, and a container affords holding, regardless of whether these parts belong to a mug, a pot, or a novel kitchen gadget. This part-based reasoning is fundamental to generalization, allowing an agent to compose known part-level skills to interact with a virtually infinite variety of unseen objects.

% The formalization of this idea in robotics was significantly advanced by the concept of Generalizable and Actionable Parts (GAParts), introduced in GAPartNet~\cite{geng2023gapartnet}. This work established a large-scale dataset and a clear taxonomy for parts that are not only visually similar across different object categories (generalizable) but also share consistent manipulation strategies (actionable). By defining canonical coordinate frames and interaction semantics for classes like `hinge doors' or `line handles,' GAPartNet provided a foundational vocabulary for part-based affordance learning. Building upon this, PartManip~\cite{geng2023partmanip} demonstrated how to learn cross-category manipulation policies by first training a state-based expert with access to ground-truth part information and then distilling this knowledge into a vision-based student that operates on raw point clouds. This progression illustrates a concrete pathway from conceptual part definitions to learned, vision-driven manipulation skills.

% The utility of part-based understanding is greatly amplified when connected to natural language, enabling robots to perform more fine-grained, instruction-driven tasks. While manipulating a `handle' is a primitive skill, following a command like `pick up the bottle and show me the cap' requires a deeper reasoning about the relationship between parts and the user's intent. The PartInstruct benchmark~\cite{yin2025partinstruct} was created to drive research in this direction, providing a large-scale dataset of part-level instructions and expert demonstrations for complex, multi-step tasks. Concurrently, works like 3DAPNet~\cite{nguyen2024language} have focused on grounding open-vocabulary language labels (e.g., `grasp to pour') directly to specific part regions and their corresponding 6-DoF interaction poses, effectively creating a language-conditioned affordance-pose detector.

% Beyond recognizing and acting on individual parts, a more advanced form of compositional reasoning involves decomposing entire actions into a set of relationships between parts. Composable Part-based Manipulation (CPM)~\cite{liu2023composable} introduces the novel idea that a functional action can be represented as a composition of part-part functional correspondences. For example, the `pouring' action is not a monolithic skill but a combination of constraints:
% align, rim\_source, rim\_target, tilt, body\_source, body\_target, and facing-up, handle\_source, body\_target.
% CPM employs a collection of composable diffusion models, each trained to capture a primitive correspondence. At inference time, these models are combined to generate manipulation parameters that satisfy all constraints simultaneously. This approach provides a powerful generative framework for manipulation, enabling zero-shot generalization to novel object categories by composing learned, primitive part-level relationships. This shift from part-centric affordances to inter-part relations represents a significant step towards a more flexible and unified understanding of manipulation.



% \subsection{Spatial Affordance}

% While understanding the affordances of individual objects is crucial, intelligent manipulation in unstructured environments requires reasoning that extends beyond the object to the scene itself. This gives rise to the concept of spatial affordance, which concerns the interactive possibilities defined by the spatial layout of a scene and the relationships between its entities. It addresses questions not of what an object can do, but where an action can take place—where an item can be placed, which gap can be traversed, or how objects can be arranged relative to one another. A unified understanding of manipulation must therefore account for this contextual, scene-level reasoning.

% A primary challenge has been that standard VLMs, trained on internet-scale 2D image-caption pairs, inherently lack a robust understanding of 3D space. Foundational work has thus focused on injecting this basic spatial knowledge into VLMs through large-scale data synthesis. Frameworks like SpatialVLM~\cite{chen2024spatialvlm} and SpatialBot~\cite{cai2025spatialbot} pioneered this data-centric approach. By leveraging off-the-shelf vision models (e.g., for metric depth estimation) to lift 2D images into 3D, they automatically generated massive Visual Question Answering (VQA) datasets. Training on these datasets, which contain millions of questions about metric distances, sizes, and relative positions, endows VLMs with a foundational vocabulary for spatial reasoning.

% With this basic vocabulary established, the next step is to tailor spatial understanding for robotic action. The ROBO SPATIAL~\cite{song2025robospatial} benchmark was designed for this purpose, defining three core categories of robotics-relevant spatial queries: spatial configuration (e.g., "Is the mug to the left of the laptop?"), spatial compatibility (e.g., "Can the chair fit in front of the table?"), and spatial context (e.g., "Point to a vacant space on the counter."). Critically, this work emphasizes the importance of reasoning across multiple reference frames—ego-centric, world-centric, and object-centric—a capability essential for any embodied agent that must interpret commands from different perspectives.

% Even with a conceptual understanding of where an action is possible, a robot requires a precise target for execution. A significant leap in bridging high-level reasoning and low-level control has been the move towards precise, point-based outputs. RoboPoint~\cite{yuan2025robopoint} trains a VLM to predict a specific pixel coordinate as a "spatial affordance point" that directly grounds a language instruction. Instead of outputting a text answer, the model points to the exact location where an action, such as placing or grasping, should occur. This directly translates abstract spatial language into an actionable target. A parallel line of work, Robotic Visual Instruction (VIEW)~\cite{li2025robotic}, addresses the precision problem from the input side, proposing a paradigm where users communicate spatial intent through unambiguous, hand-drawn sketches like arrows and circles, which are then decoded into robot actions.

% Ultimately, a robust and generalizable spatial understanding system must flexibly integrate diverse forms of spatial information. Recent work has begun to analyze the spectrum of spatially-grounded mid-level representations that bridge high-level perception and low-level action~\cite{yang2025bridging}. This research categorizes representations along dimensions such as object-centricity, motion-centricity, pose-awareness, and depth-awareness, finding that different manipulation tasks benefit from different types of grounding. To leverage this insight, they propose a Mixture-of-Experts (MoE) policy architecture that dynamically combines multiple specialized models, each trained on a distinct mid-level representation. This approach acknowledges that there is no single "best" spatial representation; rather, a unified understanding emerges from the ability to synthesize the right spatial information for the task at hand. This progression—from learning basic spatial concepts to reasoning about actionable possibilities and finally to flexibly combining precise, multi-faceted spatial representations—is critical for enabling robots to operate intelligently and reliably in complex human environments.



% \subsection{Visual Affordance}
% Visual affordance learning serves as the critical bridge connecting raw perceptual input to executable robot actions. It is fundamentally a grounding problem: how to transform high-dimensional sensor data, such as pixels or point clouds, into a representation that encodes interaction possibilities. The evolution of visual affordance representations—from dense spatial maps to sparse keypoints, and from static 2D views to dynamic 3D understanding—charts a clear path towards a more unified and capable framework for robot manipulation.

% A foundational paradigm in this area was established by Transporter Networks~\cite{zeng2021transporter}, which reformulated manipulation as a visual correspondence problem. By learning dense, pixel-aligned feature maps from top-down orthographic images, this approach could predict affordance heatmaps for "picking" and "placing" through spatial feature matching (cross-correlation). The inherent SE(2) equivariance of this formulation made it remarkably data-efficient and established a powerful "where" pathway for action, grounding manipulation directly in the visual space without explicit object models.

% While spatially precise, this initial paradigm lacked semantic understanding. The subsequent integration of pre-trained vision-language models (VLMs) was a pivotal step. CLIPort~\cite{shridhar2022cliport} ingeniously combined the semantic prowess of CLIP with the spatial accuracy of Transporter Networks, introducing a two-stream architecture. A semantic "what" pathway interprets the language instruction, while a spatial "where" pathway identifies the precise location for interaction. This decoupling of "what" and "where" proved highly effective. Further research demonstrated that such visual affordance maps need not rely solely on expert demonstrations; they can be learned in a self-supervised manner from unstructured "play" data, as shown by VAPO~\cite{borjadiaz2022affordance}, and can be used to guide hierarchical policies, as in HULC++~\cite{mees2023grounding}.

% Despite their success, dense heatmaps can lack the precision required for fine-grained tasks. This led to a shift towards sparser, more object-centric representations. KITE~\cite{sundaresan2023kite} championed this shift by grounding language instructions not to a dense map, but to a discrete set of 2D keypoints. This representation offers superior precision and cleanly decouples the problem into a grounding module, which identifies the exact point of interaction, and an acting module, which executes a keypoint-conditioned skill. This focus on sparse, semantically meaningful points marked a significant refinement in visual affordance representation.

% Furthermore, most early methods were constrained by their reliance on canonical, often top-down, 2D camera views, limiting their applicability in mobile manipulation. SLAP~\cite{parashar2023spatiallanguageattentionpoliciesefficient} addressed this by transitioning the visual input modality from 2D images or voxels to 3D point cloud "tokens". This inherently view-invariant representation allows the policy to reason about affordances from arbitrary, egocentric viewpoints, a crucial capability for robots operating in dynamic, real-world environments.

% More recently, the role of foundation models has evolved from passive feature extractors to active reasoning engines that communicate visually. This is exemplified by the paradigm of visual prompting. MOKA~\cite{liu2024moka} introduced a method where a VLM generates explicit visual "marks" (e.g., colored dots) on an image to unambiguously guide a low-level policy. Taking this a step further, PIVOT~\cite{nasiriany2024pivot} proposed an iterative process where a VLM suggests a visual action, a verifier assesses its feasibility, and the VLM refines its proposal based on the feedback. This transforms visual affordance prediction from a single-shot inference into a closed-loop, deliberative reasoning process.


\subsection{Affordance Learning}
\label{sec:affordance_learning}

A unified understanding of robot manipulation requires moving beyond asking \textit{what} things are to discerning \textit{what can be done} with them. The concept of affordance, originating from psychologist J.J. Gibson, provides a powerful framework for this shift~\cite{gibson2014theory}. In robotics, an affordance represents the potential for interaction an object or environment offers relative to an agent's capabilities—a door affords opening, a surface affords placing. By intrinsically linking perception to action, affordances serve as a foundational bridge for building more general and intelligent manipulation systems.

The study of affordances has evolved from early model-based geometric reasoning to modern data-driven paradigms. The rise of deep learning, in particular, now enables robots to learn functional properties directly from raw sensory data, often through self-supervised interaction or by leveraging the vast knowledge embedded in foundation models. This chapter explores the central role of affordance in this modern context, dissecting the concept from four critical perspectives based on the primary source of information: geometric, visual, semantic, and multimodal.

\subsubsection{Geometric Affordance}
\label{subsec:geometric_affordance}

Geometric affordance posits that an object's functional possibilities are fundamentally dictated by its three-dimensional shape, structure, and kinematics. Research in this area often focuses on inferring an object's kinematic model—its parts, joints, and movement constraints—directly from its 3D geometry~\cite{jiang2022ditto, geng2023gapartnet, geng2023partmanip}. For example, interactive approaches like Ditto~\cite{jiang2022ditto} discover articulation models by physically probing an object and observing its response.

A key principle for generalizing geometric affordances is \textit{compositionality}, where the function of a complex object is understood as the sum of its functional parts~\cite{geng2023gapartnet, geng2023partmanip, liu2023composable}. Landmark efforts such as GAPartNet~\cite{geng2023gapartnet} established taxonomies of cross-category parts, enabling policies to learn skills for ``any handle'' rather than ``a specific mug's handle''. More advanced frameworks like CPM~\cite{liu2023composable} take this further by representing complex actions not as monolithic skills, but as a composition of geometric constraints between the constituent parts of interacting objects.

\subsubsection{Visual Affordance}
\label{subsec:visual_affordance}

Visual affordance focuses on directly learning interaction possibilities from 2D visual data, such as RGB or RGB-D images. This paradigm typically formulates manipulation as a visual correspondence problem, learning to produce dense, pixel-wise affordance maps that indicate where an action can be performed~\cite{zeng2021transporter, borjadiaz2022affordancelearningplaysampleefficient, geng2022endtoendaffordancelearningrobotic, tang2025functofunctioncentriconeshotimitation, kim2025screwsplatendtoendmethodarticulated}.

The seminal Transporter Networks~\cite{zeng2021transporter} established this approach by using a spatially equivariant architecture to predict pick-and-place heatmaps via feature matching. This powerful ``where'' pathway grounds manipulation directly in the pixel space without needing explicit object models. The scalability of this idea was later enhanced by methods like VAPO~\cite{borjadiaz2022affordancelearningplaysampleefficient}, which demonstrated that such visual affordance maps could be learned in a self-supervised manner from unstructured ``play'' data, significantly reducing the reliance on expert demonstrations.

\subsubsection{Semantic Affordance}
\label{subsec:semantic_affordance}

Semantic affordance explores the connection between high-level, symbolic concepts and an agent's actions. Before the widespread adoption of modern foundation models, this line of research focused on how human-defined semantic labels, such as object categories or part names, could guide robot behavior. This perspective represents an early effort to bridge symbolic reasoning with physical interaction, providing a historical context for the multimodal approaches that dominate the field today.

For example, pioneering research in affordance-based imitation learning~\cite{4399517} investigated how a robot could learn to manipulate objects by associating semantic properties with observed human actions. By identifying object parts like ``handles'' or ``lids'' and linking them to specific manipulation trajectories, the robot could generalize its learned skills to new objects that shared similar semantic attributes. While often limited by the need for pre-defined semantic categories, these methods established the critical principle that abstract, human-understandable knowledge is a powerful prior for guiding robot learning.

\subsubsection{Multimodal Affordance}
\label{subsec:multimodal_affordance}

The current frontier of affordance learning lies in the fusion of multiple information modalities, driven by the powerful reasoning and grounding capabilities of Vision-Language Models (VLMs) and Large Language Models (LLMs). This multimodal perspective moves beyond any single source of information, aiming to create a holistic understanding of interaction potential by synthesizing visual appearance, linguistic instruction, spatial context, and geometric structure.

A dominant research thrust is the fusion of natural language with visual perception, allowing robots to ground high-level instructions in the scene~\cite{shridhar2022cliport, mees2023grounding, yin2025partinstruct, geng2024sage, huang2025a3vlm}. Landmark architectures like CLIPort~\cite{shridhar2022cliport} introduced a two-stream model, effectively creating a semantic "what" pathway to interpret language and a spatial "where" pathway to localize the action. This principle has been extended to ground language to ever-finer details, such as specific object parts~\cite{yin2025partinstruct, geng2024sage}.

Another critical fusion involves endowing models with an explicit understanding of 3D space, enabling them to reason about metric properties like distance, orientation, and layout~\cite{chen2024spatialvlm, cai2025spatialbot, song2025robospatial, yuan2025robopoint}. To make this spatial understanding directly actionable, methods like RoboPoint~\cite{yuan2025robopoint} train models to output a precise pixel coordinate as a "spatial affordance point," translating abstract spatial language into a concrete target.

Furthermore, the interaction paradigm itself is evolving into a multimodal dialogue, incorporating new input modalities and enabling models to reason and recover from failure~\cite{liu2024moka, li2025robotic, huang2024copageneralroboticmanipulation, xiong2025autonomous}. For instance, visual prompting approaches like MOKA~\cite{liu2024moka} allow a VLM to generate explicit visual ``mark'' on an image to unambiguously guide a policy, while frameworks like AIC-MLLM~\cite{xiong2025autonomous} enable the model to learn from its own failures through interactive correction.

Finally, a key goal is to learn unified and generalizable affordance representations that transfer to novel objects and tasks~\cite{yu2025uniaff, tang2025uad, kuang2025ram}. This is pursued by learning unified representations for diverse object types, such as tools and articulated objects~\cite{yu2025uniaff}, or by developing methods for unsupervised or retrieval-based affordance transfer to unseen objects~\cite{tang2025uad, kuang2025ram}. This convergence of modalities is paving the way for robots that can reason about and act upon a much richer and more nuanced understanding of the world.


\subsection{3D Representation as Planner}
Although 3D representations such as Gaussian Splatting and Neural Descriptor Fields do not directly produce control signals, they function as planning modules by generating structured action proposals (e.g., 6-DoF grasps, relational rearrangements, or optimization costs). In this sense, they serve as mid-level planners that bridge perception and action, and are therefore included under the high-level planning category.

Recent work on manipulation has converged on mid-level 3D scene representations that turn perception into actionable proposals (e.g., 6-DoF grasps, keyframes, or cost fields) rather than full task plans. Two trends drive this line: (i) editable, real-time Gaussian splatting (GS) variants that fuse geometry with semantics/motion and enable scene editing, and (ii) implicit/descriptor fields that distill features from 2D foundation models into 3D for correspondence and language grounding.

\textbf{Gaussian-splatting scene representations and editing.}
Splat-MOVER builds a modular stack (ASK/SEE/Grasp-Splat) for open-vocabulary manipulation by distilling semantics/affordances into a 3DGS “digital twin,” then proposing grasp candidates for planning~\cite{shorinwa2025splat}. 
Object-Aware GS adds object-centric, 30 Hz dynamic reconstruction with semantics~\cite{li2024object}. 
Physically Embodied GS couples particles (physics) to 3DGS (vision) for a real-time, visually-correctable world model~\cite{abou2025physically}. 
MSGField uses 2DGS with attached motion/semantic attributes for language-guided manipulation in dynamic scenes~\cite{sheng2024msgfield}. 
RoboSplat directly edits 3DGS reconstructions to synthesize diverse demonstrations (objects, poses, views, lighting, embodiments), substantially boosting one-shot visuomotor policy generalization~\cite{yang2025novel}.

\textbf{Implicit/descriptor fields.}
NDF learns SE(3)-equivariant descriptors for few-shot pose transfer~\cite{simeonov2022neural}; R-NDF extends to relational rearrangement across objects~\cite{simeonov2023se}; F3RM distills CLIP features into 3D fields for few-shot, language-conditioned grasp/place~\cite{shen2023distilled}; $D^3$Fields builds dynamic 3D descriptor fields that support zero-shot rearrangement via image-specified goals~\cite{wang2025d}.

\textbf{Generative world models.}
Imagination Policy “imagines” target point clouds and converts them to keyframe actions via rigid registration—turning action inference into a local generative task with strong real-robot result~\cite{huang2025imagination}.

\textbf{Structured scene graphs.}
RoboEXP incrementally constructs an action-conditioned scene graph (ACSG) via interactive exploration, enriching the state with action-relevant relations for downstream manipulation~\cite{jiang2025roboexp}.

==> tables/8_applications/application.tex <==
\begin{table}[ht]
\label{tab: app}
\centering
\caption{Applications of Robotic Manipulation.}
\begin{tabular}{lllll}
\toprule
\textbf{Area} & \textbf{Task Example} &  \textbf{Task Description} & \textbf{Applicable Model} \\
\midrule
\multirow{5}{*}{Household Robots}  
  & Object rearrangement & Putting household items back to their designated places. & e.g., Stable Diffusion \cite{jin2025paca} \\
  & Surface cleaning & Wiping or tidying flat surfaces such as tables or counters. & e.g., VLA \cite{li2025hamster}  \\
  & Laundry folding & Folding clothes using two-handed manipulation. & e.g., LLAMA \cite{chen2025metafold}\\
\midrule
\multirow{5}{*}{Industrial Robots}  
  & Human-robot collaboration & Assisting humans in flexible manufacturing tasks. & e.g., DNN \cite{liu2018deep} \\
  & Robot assembly & Learning to assemble components in structured tasks like peg-in-hole. & e.g., DQN\cite{li2022flexible} \\
  & Mobile Manipulation & Performing complex tasks involving both navigation and object interaction. & e.g., VLA\cite{wu2025momanipvla} \\
  \midrule
  \multirow{5}{*}{AI4Science}  
  & Medical Science & Assisting in medical tasks, e.g., surgery. & e.g., VLA \cite{he2025capsdt} \\
  & Physical Science & Assisting in physical tasks, e.g., sports  & e.g.,  SNN \cite{wang2025spikepingpong}\\
  & Chemical Science & Assisting in chemical tasks, e.g., chemical research. & e.g., LLAMA \cite{song2025multiagent}\\
  \midrule
  \multirow{5}{*}{Agriculture}  
  & Robotic planting and seeding & Automating the process of planting seeds in agricultural fields.  & e.g., VLA \cite{sapkota2025vision} \\
  & Robotic harvesting & Automating the detection and picking of crops using robotic system & e.g.,  Detection network \cite{alaaudeen2024intelligent}\\
& Robotic weeding & Identifying and removing weeds using vision-guided robotic systems & e.g., YOLOX \cite{zhu2022yolox} \\
\bottomrule
\end{tabular}
\end{table}

% a r
